Latent SDEs on Homogeneous Spaces

We consider the problem of variational Bayesian inference in a latent variable model where a (possibly complex) observed stochastic process is governed by the solution of a latent stochastic differential equation (SDE). Motivated by the challenges that arise when trying to learn an (almost arbitrary) latent neural SDE from data, such as efficient gradient computation, we take a step back and study a specific subclass instead. In our case, the SDE evolves on a homogeneous latent space and is induced by stochastic dynamics of the corresponding (matrix) Lie group. In learning problems, SDEs on the unit n-sphere are arguably the most relevant incarnation of this setup. Notably, for variational inference, the sphere not only facilitates using a truly uninformative prior, but we also obtain a particularly simple and intuitive expression for the Kullback-Leibler divergence between the approximate posterior and prior process in the evidence lower bound. Experiments demonstrate that a latent SDE of the proposed type can be learned efficiently by means of an existing one-step geometric Euler-Maruyama scheme. Despite restricting ourselves to a less rich class of SDEs, we achieve competitive or even state-of-the-art results on various time series interpolation/classification problems.

==> figs/path_on_sphere/rotate.tex <==
\def\axlen{1.5}
\def\rad{1}
\begin{tikzpicture}
	\pgfmathsetmacro{\CameraX}{sin(\ViewAzimuth)*cos(\ViewElevation)}
	\pgfmathsetmacro{\CameraY}{-cos(\ViewAzimuth)*cos(\ViewElevation)}
	\pgfmathsetmacro{\CameraZ}{sin(\ViewElevation)}
	%\path[use as bounding box] (-\rad,-\rad) rectangle (\rad,\rad); % Avoid jittering animation
	
	% Draw a nice looking sphere
		\clip (0,0) circle (\rad);
		\begin{scope}[transform canvas={rotate=-20}]
			\shade[shading=goodsphere] (0,0) circle (\rad);
		\end{scope}
	\begin{axis}[
		at = {(0,0)},
		hide axis,
		view={-10}{18},     % Set view angle
		every axis plot/.style={very thin},
		disabledatascaling,                      % Align PGFPlots coordinates with TikZ
		anchor=origin,                           % Align PGFPlots coordinates with TikZ
		viewport={-10}{18}, % Align PGFPlots coordinates with TikZ
		viewport={-10}{18}, % Align PGFPlots coordinates with TikZ
		rotate around x = 0, rotate around y = 30, rotate around z=0
		]
		\foreach \t in {0,45,...,180}
		\addFGBGplot[domain=0:2*pi, samples=100, samples y=1, color=gray] (\rad*cos(\t)*sin(deg(x)), {\rad*sin(\t)*sin(deg(x))}, {\rad*cos(deg(x))});
		\draw[] (axis cs:0, 0,-\axlen*\rad) -- (axis cs:0,0,-1.2*\rad);
		\draw[<-] (axis cs:0, 0,\axlen*\rad) -- (axis cs:0,0,1.2*\rad);
		\addplot3 [green!20!black, only marks] coordinates {
        (0,-1*\rad,0)
    }; 
	\end{axis}
\end{tikzpicture} 

==> figs/path_on_sphere/tikzmacros.tex <==
\pgfplotsset{compat=1.15}
\definecolor{shadecolor}{HTML}{000000}
\def\rad{2}
\def\shadeangle{90}
\newcommand{\ViewAzimuth}{0}
\newcommand{\ViewElevation}{0}
% Style to select only points from #1 to #2 (inclusive)
\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}
\pgfdeclareradialshading{goodsphere}{\pgfpoint{-15}{12bp}}{%
  color(0bp)=(black!0);
  color(2.5bp)=(black!0.5);
  color(5bp)=(black!2);
  color(7.5bp)=(black!4);
  color(10bp)=(black!8.3);
  color(12.5bp)=(black!13.3);
  color(15.bp)=(black!20);
  color(17.5bp)=(black!28.6);
  color(20bp)=(black!40);
  color(22.5bp)=(black!56);
  color(23.75bp)=(black!68.8);
  color(24.375bp)=(black!77.8);
  color(25bp)=(black!85.9);
  color(30bp)=(black)
}
% Declare nice sphere shading: http://tex.stackexchange.com/a/54239/12440
\pgfdeclareradialshading[tikz@ball]{ball}{\pgfqpoint{0bp}{0bp}}{%
	color(0bp)=(tikz@ball!0!white);
	color(3bp)=(tikz@ball!10!white);
	color(15bp)=(tikz@ball!70!black);
	color(20bp)=(shadecolor!70);
	color(25bp)=(shadecolor!70);
	color(30bp)=(shadecolor!70)}
\pgfdeclarefunctionalshading{eightball}{\pgfpointorigin}{\pgfpoint{100bp}{100bp}}{}{
		% Compute distance difference (horizontally weighted twice). (50bp,50bp) is the center
		65 sub dup mul exch               %Change the coordinate to move vertically
		40 sub dup mul 0.5 mul add sqrt   %Change the coordinate to move horizontally
		% In MATLAB notation : d=distance diff
		% x=1.003^(-d^2)
		dup mul neg 1.003 exch exp
		% x is the only variable in the stack now but we need 3 values at the top of the stack
		% so we duplicate these values putting new values in the stack.
		dup % Duplicates with the current value and pushes the stack down (value of green)
		dup % Duplicates with the current value and pushes the stack down (value of blue)
		}
		\pgfdeclarefunctionalshading{sphere}{\pgfpoint{-25bp}{-25bp}}{\pgfpoint{25bp}{25bp}}{}{
			%% calculate unit coordinates
			25 div exch
			25 div exch
			%% copy stack
			2 copy 
			%% compute -z^2 of the current position 
			dup mul exch
			dup mul add
			1.0 sub
			%% and the -z^2 of the light source 
			0.3 dup mul
			-0.5 dup mul add
			1.0 sub
			%% now their sqrt product
			mul abs sqrt
			%% and the sum product of the rest
			exch 0.3 mul add
			exch -0.5 mul add
			%% max(dotprod,0)
			dup abs add 2.0 div 
			%% matte-ify
			0.6 mul 0.4 add
			%% currently there is just one number in the stack.
			%% we need three corresponding to the RGB values
			dup
			dup
			}

\makeatletter
\newcommand{\gettikzcoordinates}[3]{%
	\tikz@scan@one@point\pgfutil@firstofone#1\relax
	\pgfmathsetmacro{\myx}{round(0.99626*\the\pgf@x/0.0283465)/1000}
	\pgfmathsetmacro{\myy}{round(0.99626*\the\pgf@y/0.0283465)/1000}
	\pgfmathsetmacro{\myz}{round(0.99626*\the\pgf@z/0.0283465)/1000}
	\global\edef#2{(\myx,\myy,\myz)}%
}
\makeatother

% Style to set TikZ camera angle, like PGFPlots `view`
\tikzset{viewport/.style 2 args={
		x={({cos(-#1)*1cm},{sin(-#1)*sin(#2)*1cm})},
		y={({-sin(-#1)*1cm},{cos(-#1)*sin(#2)*1cm})},
		z={(0,{cos(#2)*1cm})}
}}

% Styles to plot only points that are before or behind the sphere.
\pgfplotsset{only foreground/.style={
		restrict expr to domain={rawx*\CameraX + rawy*\CameraY + rawz*\CameraZ}{-0.05:100},
}}
\pgfplotsset{only background/.style={
		restrict expr to domain={rawx*\CameraX + rawy*\CameraY + rawz*\CameraZ}{-100:0.05}
}}

% Automatically plot transparent lines in background and solid lines in foreground
\def\addFGBGplot[#1]#2;{
	\addplot3[#1,only background, opacity=0.25] #2;
	\addplot3[#1,only foreground] #2;
}

\pgfplotsset{select coords between index/.style 2 args={
    x filter/.code={
        \ifnum\coordindex<#1\def\pgfmathresult{}\fi
        \ifnum\coordindex>#2\def\pgfmathresult{}\fi
    }
}}

\newcommand{\drawpath}[4]{
	% draw origin to align plot with sphere
	\addplot3[
		mark=none,
		line width = .5,
		]  coordinates {
			(0,0,0) };
	\addplot3[
		color=#3,
		only marks,
		,mark options={draw=#4, fill=#4, scale=1},
		select coords between index = {0}{0}
		] table [
			x expr = \thisrowno{0}*#2,
			y expr = \thisrowno{1}*#2,
			z expr = \thisrowno{2}*#2,
			col sep=comma
			]  {#1};
	\addplot3[
	color=#3,
	mark=none,
	line width = .5,
	] table [
		x expr = \thisrowno{0}*#2,
		y expr = \thisrowno{1}*#2,
		z expr = \thisrowno{2}*#2,
		col sep=comma
		]  {#1};
}

==> figs/plate.tex <==
\begin{tikzpicture}[scale=1, transform shape]
    \node[obs] (x1) {$\mathbf{x}$};
    \node[latent, above=of x1] (z1) {$\mathbf{z}$};
    \node[const, left=of z1] (phi1) {$\boldsymbol{\phi}$};
    \node[const, right=of z1] (theta1) {$\boldsymbol{\theta}$};
    \path[dashed,-latex] (phi1) edge (z1);

    %helper noes for positioning
    \node[below=of z1, xshift=.45cm, yshift=-.75cm] (h1) {$N$};

    %\edge [dashed] {phi1} {z1};
    \edge {theta1} {z1};
    \edge {theta1.south west} {x1};
    \draw (x1) edge[out=135,in=225,-latex,dashed] (z1);
    %
    \edge {z1} {x1};
    \plate[xscale=1.5] {xz} {(x1)(z1)} {\phantom{$N$}};
\end{tikzpicture}
